PanDORA: Casual HDR Radiance Acquisition of Indoor Scenes for Image-based Lighting

Most novel view synthesis methods -- including Neural Radiance Fields (NeRF) -- struggle to capture the high dynamic range (HDR) radiance required for realistic image-based lighting (IBL). This limitation stems from a reliance on low dynamic range (LDR) imagery, which fails to capture the intensity of light sources found in indoor environments. While exposure bracketing can recover this range, it is often too slow for practical, large-scale acquisition. In this work, we introduce PanDORA: PANoramic Dual-Observer Radiance Acquisition, a system specifically designed for the fast and affordable capture of high-quality HDR radiance maps for IBL. Our approach utilizes two 360{\deg} cameras mounted on a portable monopod to simultaneously record videos at different exposures. These videos are processed by our proposed two-stage NeRF-based algorithm featuring a novel self-calibrating pipeline to estimate camera parameters. This pipeline produces non-saturated HDR radiance fields that accurately capture the radiance of a scene. When evaluated on a new dataset of real indoor environments featuring HDR ground truth lighting, PanDORA demonstrates superior fidelity in reconstructing the peak intensities necessary for downstream rendering tasks, providing a scalable and efficient solution for capturing real-world IBLs.

==> latexmkrc <==
#!/usr/bin/perl

#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}



## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.2;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";

